Enhancing Incremental Summarization with Structured Representations

Large language models (LLMs) often struggle with processing extensive input contexts, which can lead to redundant, inaccurate, or incoherent summaries. Recent methods have used unstructured memory to incrementally process these contexts, but they still suffer from information overload due to the volume of unstructured data handled. In our study, we introduce structured knowledge representations ($GU_{json}$), which significantly improve summarization performance by 40% and 14% across two public datasets. Most notably, we propose the Chain-of-Key strategy ($CoK_{json}$) that dynamically updates or augments these representations with new information, rather than recreating the structured memory for each new source. This method further enhances performance by 7% and 4% on the datasets.

==> sections/2-related_work.tex <==
\paragraph{LLMs with memory}

\paragraph{Incremental Summarization}

==> sections/unused.tex <==
% \begin{table*}[t]
% \scriptsize
% \centering
% \begin{tabular}{l|l|l|rrrrrrr|r}
% \toprule
%  &  & \multicolumn{7}{c}{Turns} \\

%  & Model & Metric & 1 & 2 & 3 & 4 & 5 & 6 & 7 & Avg.\\

% \toprule
% \multirow{9}{*}{GENERATE w/ JSON} & Gemini-Ultra & Precision  & - & - & - & - & - & - &  0.912 & \\
% &  & Recall & - & - & - & - & - & - & 0.589 & \\ 
% & & F1 & - & - & - & - & - & - & 0.709 & \\
%  \cmidrule{2-11}

% & GPT3.5 & Precision &  &  & &  &  &  &  & \\
% &  & Recall &  &  & &  &  &  &  & \\ 
% &  & F1 &  &  & &  &  &  &  & \\
%  \cmidrule{2-11}

% & Gemini-Pro & Precision& - & - & - & - & - & - & 0.856 & \\
% &  & Recall & - & - & - & - & - & - & 0.614 & \\ 
% &  & F1  & - & - & - & - & - & - & 0.704 & \\
  
% \bottomrule

% \toprule
% \multirow{9}{*}{UPDATE w/ TEXT} & Gemini-Ultra & Precision  & ? & ? & - & - & - & - &   & \\
% &  & Recall & - & - & - & - & - & - &  & \\ 
% & & F1 & - & - & - & - & - & - &  & \\
% &  & num tokens & 0.0 & 130.1 & 255.6 & 325.4 & 435.375 & 583.0 & 488.7 &  \\
% &  & \# attr-val pairs & - & - & - & - & - & - &  &  \\ 

%  \cmidrule{2-11}

% & GPT3.5 & Precision &  &  & &  &  &  &  & \\
% &  & Recall &  &  & &  &  &  &  & \\ 
% &  & F1 &  &  & &  &  &  &  & \\
%  \cmidrule{2-11}

% & Gemini-Pro & Precision& 0.655 & 0.650 & 0.676 & 0.748 & 0.740 & 0.751 & 0.790 & \\
% &  & Recall & 0.695 & 0.607 & 0.565 & 0.487 & 0.558 & 0.361 & 0.317 & \\ 
% &  & F1  & 0.661 & 0.612 & 0.610 & 0.571 & 0.626 & 0.464 & 0.416 & \\
% &  & num tokens & 0.0 & 130.1 & 255.6 & 325.4 & 435.375 & 583.0 & 488.7 &  \\
% &  & \# attr-val pairs & - & - & - & - & - & - &  &  \\ 
  
% \bottomrule

% \toprule
%  \multirow{9}{*}{UPDATE w/ JSON} & Gemini-Ultra & Precision & 0.903 &  0.791 & 0.778 & 0.785 & 0.808 & 0.813 & 0.813 &  \\
% &  & Recall & 0.803 & 0.791 & 0.761 & 0.721 & 0.689 & 0.602 & 0.557 &  \\ 
% & & F1 & 0.840 & 0.785 & 0.762 & 0.743 & 0.726 & 0.667 & 0.640 &  \\
% &  & num tokens & 0.0 & 100.6 & 196.1 & 278.1 & 344.4 & 401.1 & 415.4 &  \\
% &  & \# attr-val pairs & 7.2 & 10.8 & 12.6 & 13.1 & 13.5 & 12.9 & 12.7 &  \\ 
%  \cmidrule{2-11}

% & GPT3.5 & Precision &  &  &  &  &  &  &  &  \\
% &  & Recall &  &  &  &  &  &  &  &  \\ 
% &  & F1 &  &  &  &  &  &  &  &  \\

%  \cmidrule{2-11}

% & Gemini-Pro & Precision & 0.866 & 0.853 & 0.846 & 0.837  & 0.838 & 0.813 & 0.823 & \\
% &  & Recall & 0.814 & 0.745 & 0.687 & 0.635 & 0.644 & 0.563 & 0.511 &  \\ 
% &  & F1 & 0.833 & 0.786 & 0.746 & 0.711 & 0.720 & 0.646 & 0.615 &  \\
% &  & num tokens & 0.0 & 125.6 & 205.9 & 268.3 & 322.4 & 405.4 & 421.5 &  \\
% &  & \# attr-val pairs & 8.2 & 10.2 & 11.7 & 12.4 & 13.5 & 13.3 & 12.1 &  \\

% \bottomrule
% \toprule
% \multirow{9}{*}{TABLA w/ JSON} & Gemini-Ultra & Precision  & 0.915 & 0.857 & 0.840 & 0.831 & 0.847  & 0.847 & 0.848 & \\
% &  & Recall & 0.815 & 0.815 & 0.812 & 0.792 & 0.774 & 0.781 & 0.769 & \\ 
% & & F1 & 0.855 & 0.832 & 0.822 & 0.808 & 0.806 & 0.810 & 0.804 & \\
% &  & num tokens & 0.0 & 104.2 & 210.6 & 317.6 & 412.8 & 491.3 & 576.0 &  \\
% &  & \# attr-val pairs & 7.0 & 10.7 & 13.8 & 16.1 & 18.0 & 19.9 & 21.7 &  \\


%  \cmidrule{2-11}

% & GPT3.5 & Precision &  &  & &  &  &  &  & \\
% &  & Recall &  &  & &  &  &  &  & \\ 
% &  & F1 &  &  & &  &  &  &  & \\
%  \cmidrule{2-11}

% & Gemini-Pro & Precision & 0.904 & 0.858 & 0.827 & 0.817 & 0.833 & 0.796 & 0.801 & \\
% &  & Recall & 0.823 & 0.842 & 0.832 & 0.800 & 0.764 & 0.780 & 0.754 & \\ 
% &  & F1 & 0.857 & 0.842 & 0.821 & 0.801 & 0.791 & 0.785 & 0.775 & \\
%   &  & num tokens & 0.0 & 130.5 & 268.0 & 400.3 & 557.8 & 656.2 & 809.6 &  \\
% &  & \# attr-val pairs & 9.6 & 13.9 & 19.5 & 23.3 & 26.5 & 30.0 & 31.8 &  \\

% \bottomrule

% \toprule
% \multirow{9}{*}{MERGE w/ JSON} & Gemini-Ultra & Precision  & 0.895 & 0.871 & 0.860 & 0.854 & 0.861 & 0.865 & 0.856 & \\
% &  & Recall & 0.793 & 0.763 &0.719 & 0.687 & 0.680 & 0.649 & 0.621 & \\ 
% & & F1 & 0.833 & 0.808 & 0.779 & 0.758 & 0.756 & 0.737 & 0.716 & \\
% &  & num tokens & 0.0 & 102.8 & 175.0 & 226.9 & 272.8 & 318.6 & 346.0 &  \\
% &  & \# attr-val pairs & 7.1 & 11.9 & 15.8 & 18.7 & 21.5 & 23.6 & 24.8 &  \\

%  \cmidrule{2-11}

% & GPT3.5 & Precision &  &  & &  &  &  &  & \\
% &  & Recall &  &  & &  &  &  &  & \\ 
% &  & F1 &  &  & &  &  &  &  & \\
%  \cmidrule{2-11}

% & Gemini-Pro & Precision & 0.864 & 0.846 & 0.852 & 0.852 & 0.844 & 0.839 & 0.821 & \\
% &  & Recall & 0.816 & 0.825 & 0.829 & 0.790 & 0.785 & 0.772 & 0.737 & \\ 
% &  & F1 & 0.833 & 0.833 & 0.837 & 0.815 & 0.811 & 0.801 & 0.775 & \\
% &  & num tokens & 0.0 & 128.0 & 240.1 & 346.9 & 414.5 & 489.2 & 568.3 &  \\
% &  & \# attr-val pairs & 8.2 & 14.4 & 19.7 & 22.8 & 26.8 & 30.4 & 33.5 &  \\

% \bottomrule
% \end{tabular}

% \caption{Performance with \ultra, \chatgpt, and \pro models across different turns. \# attr-val pairs denote the number of attribute and value pairs in the generated summary at each turn. Best F1 scores are in \textbf{boldface}.}
% \label{tab:eval-results}
% \end{table*}


% The structured JSON format organizes information into distinct, easily accessible segments, facilitating efficient updates and retrievals. This format allows the model to effectively parse and incorporate new data while maintaining a clear understanding of the evolving narrative. 

% Our method not only enhances the contextual relevance of the information but also improves LLM's ability of retaining old information. 

% Our approach based on a structured summary enhances the LLMs' ability to track complex narratives, identify critical elements, and generate more accurate and relevant summaries, outperforming plain text baselines. 


% and can't effectively filter out these insignificant details. With GM\textsubscript{json}, this results in up to 50\% of errors related to  and up to 13\% of errors related to salience (including trivial details irrelevant to the main storyline). Although the CoK method reduces salience errors by 3\% through systematic analysis and merging, it still struggles with including insignificant story details, contributing to 49\% of entity omission errors.
% In comparison, while GU\textsubscript{text} has a higher rate of entity omission errors at 60\%, it only results in 6\% of salience errors. This indicates that the text baseline is more effective at avoiding the inclusion of trivial details in the summary.



% \paragraph{Performance across models}

% We observe that feeding all paragraphs into the model at once (GENERATE) performs better than feeding each paragraph incrementally (UPDATE). However, the GENERATE option produces significantly lower recall values compared to MERGE and TABLA.

% While the \pro model shows similar performance between TABLA and MERGE, the \ultra model achieves notably higher performance with the TABLA method compared to all other methods. This suggests that \ultra has a better reasoning ability than the \pro model, as TABLA requires reasoning to determine which row to update by comparing the existing memory with the new paragraph. Although the \pro model achieves similar overall performance to the \ultra model, we noticed many duplicate attribute-value pairs in its outputs, as indicated by the high number of attribute-value pairs in Table \ref{tab:eval-results}. This suggests that the \pro model is good at extracting all seemingly relevant attribute-value pairs, but the accuracy of these pairs is low. Consequently, the precision-recall values may be inflated due to numerous redundant true positive pairs. 



% \paragraph{Performance based on Memory token size}
% Since the number of tokens in the memory for the TABLA and MERGE methods is larger than that in the text-based representation, we limit the number of tokens that the memory can store. For the SUMIE dataset, we test with limits of 200, 300, and 400 tokens, as the text-based memory representation often reaches 400 to 500 tokens. For the Book dataset, we test with limits of 1000 and 2000 tokens, considering the model's maximum token limit is 6192 tokens. A limit of 2000 tokens is a reasonable constraint, allowing the model to accommodate another 4000 tokens as a new information and an incrementally updated summary.

% While the performance decreases when we limit the number of token size in the memory, but incrementally updated summary with a JSONfied memory representation still outperforms text memory representation by a large gap.


% \paragraph{JSON vs. Markdown}
% We compare the performance between JSON and Markdown formats. At first glance, there does not seem to be a significant performance gap between the two as input representations. However, in the Book dataset, representing the book's structure using Markdown becomes challenging due to its potential expansion to multiple depths (Characters -> Name -> Events/Motivations -> Values).

% \paragraph{Performance based on enhanced evaluation}
% Table \ref{} presents the performance results using the enhanced evaluation method, which penalizes redundant pairs in the final score on the SUMIE dataset. We find that when redundancy is penalized, \ultra performs the best, while the \pro model shows significantly lower performance.


% \begin{table}[t!]
% \small
% \centering
% \begin{tabular}{l|cc}
% \toprule
%  Method & Ultra & Pro \\
% \midrule
% Generate-Update\textsubscript{text} & 51.9 &  53.1 \\
%  Generate-Update\textsubscript{json} & 61.7 & 58.5 \\
%  Generate-Merge\textsubscript{json} & 51.4 & 61.5 \\
%  Chain-of-Key Update\textsubscript{json} & - &  - \\
% %  \midrule
% % 2000 & GU\textsubscript{text} & 50.7 &  52.4 \\
% %  & GU\textsubscript{json} & 57.8 &  \\
% %  & GM\textsubscript{json} & 54.9 & 66.7 \\
% %  & CoK\textsubscript{json} & - &  - \\
 
% \bottomrule
% \end{tabular}
% \caption{BookScore accuracy with text-based memory representation and json-based memory representation on UPDATE, MERGE, and TABLA methods.
% }
% \label{tab:eval-results-book}
% \end{table}



% \begin{table}[t!]
% \scriptsize
%     \centering
% \begin{tabular}{lccc}
% \toprule
%  \bf Error types & GU\textsubscript{text} & GU\textsubscript{json} & CoK\textsubscript{json} \\
% \midrule
% entity omission & 60 & 48 & 0.48 \\
% causal omission & 19 & 25 & 0.16 \\
% event omission & 15 & 15 & 0.19 \\
% salience & 6 & 9 & 0.15 \\
% inconsistency & 0 & 1 & 0.01 \\
% discontinuity & 27 & 1 & 0.01\\
% duplication & 0 & 1 & 0.00 \\
% language & 0 & 0 & 0.00 \\

% \bottomrule
% \end{tabular}
% \caption{Error distribution (\%) for BookScore dataset using GU and CoK methods.}
% \vspace{-1em}
% \label{tab:errors-bookscore}
% \end{table}

